FILO: FIx-LOcus Localization for Backward Incompatibilities Caused by Android Framework Upgrades

Mobile operating systems evolve quickly, frequently updating the APIs that app developers use to build their apps. Unfortunately, API updates do not always guarantee backward compatibility, causing apps to not longer work properly or even crash when running with an updated system. This paper presents FILO, a tool that assists Android developers in resolving backward compatibility issues introduced by API upgrades. FILO both suggests the method that needs to be modified in the app in order to adapt the app to an upgraded API, and reports key symptoms observed in the failed execution to facilitate the fixing activity. Results obtained with the analysis of 12 actual upgrade problems and the feedback produced by early tool adopters show that FILO can practically support Android developers.FILO can be downloaded from https://gitlab.com/learnERC/filo, and its video demonstration is available at https://youtu.be/WDvkKj-wnlQ.

==> Related_Work.tex <==
\section{Related Work}
\label{sec:relatedWork}
